Normal approximation for Gibbs processes via disagreement couplings

This work improves the existing central limit theorems (CLTs) for geometric functionals of Gibbs processes in three aspects. First, we derive a CLT for weakly stabilizing functionals, thereby improving on the previously used assumption of exponential stabilization. Second, we show that this CLT holds for interaction ranges up to the percolation threshold of the dominating Poisson process. This avoids imprecise branching bounds from graphical construction. Third, by constructing simultaneous couplings of several Palm processes for Gibbs functionals, we provide a quantitative CLT in terms of Kolmogorov bounds for normal approximation. An important conceptual ingredient in these advances is the extension of disagreement coupling adapted to unbounded windows and to the comparison at multiple spatial locations.

==> ytty.tex <==
\section{Disagreement coupling for discrete Gibbs processes}
\label{sec:dis}

Let $G = (V, E)$ be a dependency graph and $\XX = \{\XX_v\}_{v \in V}$ be a $\{0, 1\}$-valued Gibbs process.  We henceforth suppose a uniform upper bound on the conditional probabilities in the sense that $\P\big(\XX_v = 0 \ba \XX_{\pa v}\big)\ge q_0$ almost surely for some $q_0 \le 1$. Then, we define an augmented Gibbs process $\XX^*$ on the extended state space $\{0_-, 0_+, 1\}$ by specifying the conditional densities 
$$\k^*_v(\s \ba  \bs{\s}_{\hat v}) := \P\big(\XX^*_v = \s \ba \XX^*_{\pa v} = \vec {\s}\big)$$
as follows
$$
\k^*_v(\s \ba  \bs{\s}_{\hat v}) =
\begin{cases}
	q_0 &\text{ if }\s = 0_-,\\
	\k(0 \ba \pi(\bs{\s}_{\hat v})) - q_0&\text{ if }\s = 0_+,\\
	\k(1 \ba \pi(\bs{\s}_{\hat v}))  &\text{ if }\s = 1,
\end{cases}
$$
where $\pi(0_-):=\pi(0_+) :=0$ and $\pi(1) := 1$. 

Now, the key observation is that when conditioning $\XX^*$ on the set $V_- := \{v\in V\co \XX^*_v = 0_-\}$, we obtain a Gibbs process $\XX'$ whose conditional densities are described in the following auxiliary result.

\bel[Conditional densities of $\XX'$]
\label{lem:cde}
Let $\XX'$ be the process $\XX^*$ conditioned on $V_-$. Then, $\XX'$ is a Gibbs process with conditional density $\k'_v$ such that if $v \in V_-$, then $\k'_v(0_- \ba \bs{\s}_{\hat v}) = 1$, and if $v \not\in  V_-$, then 
$$
\k'_v(\s \ba  \bs{\s}_{\hat v}) =
\begin{cases}
	(\k(0 \ba \pi(\bs{\s}_{\hat v})) - q_0)/p_0&\text{ if }\s = 0_+,\\
	\k(1 \ba \pi(\bs{\s}_{\hat v}))/p_0  &\text{ if }\s = 1,
\end{cases}
$$
\enl
\bep
We only need to deal with the case where $v \not \in V_-$. Moreover, since then $\XX'_v$ can only take the two values $0_+$ or 1, it suffices to verify the asserted expression for the conditional density $\k'_v(\s \ba  \bs{\s}_{\hat v})$ when $\s = 1$. To that end, we let $A \su V \sm \{v\}$ and $\bs\s \in \{0_-, 0_+, 1\}$. Then, by the spatial Markov property,
\begin{align*}
	&\P\big(\XX^*_v = 1, \XX^*_{\hat v} = \bs\s_{\hat v}, V_-\sm\{v\} = A\big) \\
	&\quad =\k(1 \ba \pi(\bs{\s}_{\hat v}))\P\big(\XX^*_{\pa v} = \bs\s_{\pa v}, V_-\sm\{v\} = A\big)
\end{align*}
and similarly,
\begin{align*}
	&\P\big(\XX^*_v \in\{0_+, 1\}, \XX^*_{\hat v} = \bs\s_{\hat v}, V_-\sm\{v\} = A\big) \\
	&\quad =p_0 \P\big(\XX^*_{\hat v} = \bs\s_{\hat v}, V_-\sm\{v\} = A\big).
\end{align*}
Hence, taking the ratio of the two expressions concludes the proof.
\enp

Suppose now that $G := G_n := [-n, n]^d \cap \Z^d$  is the discrete $2n$-cube.  Then, Lemma \ref{lem:cde} provides a specific coupling between the Gibbs processes $\XX(n)$ on $G_n$ provided that $p_0 < p_c(d)$ is smaller than the critical percolation probability on $\Z^d$.
. Indeed, we first define the limiting augmented process $\XX^*(\ff)$ as follows. First, we realize $V_-(\ff)$ as Bernoulli percolation process with marginal probability $p_0$ on $\Z^d$. Next, we define $\XX^*(\ff)$ on each of the clusters $C_i$ of $\Z^d \sm V_-(\ff)$ independently conditioned on $V_-(\ff)$ according to the conditional density given in \eqref{lem:cde}. Having constructed the limiting process $\XX^*(\ff)$, we now construct the augmented coupled processes $\XX^*(n)$ on $G_n$. 

First, we let $V_{-, n} := V_- \cap [-n, n]^d$ be the location of all sites satisfying $\XX_v(n)^* = 0_-$. Next, for each connected component $C_i$ of $\Z^d\sm V_-(\ff)$ such that $C_i$ together with its boundary is entirely contained in $[-n, n]^d$, we set $\XX_{C_i}^*(n) := \XX_{C_i}^*(\ff)$. Finally, let $R \su V_n\sm V_{-, n}$ denote the remaining sites, which are not contained in one of the components $C_i$ as just described. Then, to define $\XX_R^*(n)$, we take a sample from the conditional distribution $\P\big(\XX_R^* \in \cdot \ba \XX_{V_n \sm R}^*, V_{-,n}\big)$. To summarize, we have thus defined coupled processes $\XX^*(n)$ on $G_n$ for every $n \ge 1$ such that with probability 1, for every bounded $A \su \Z^d$ the restricted processes $\XX^*_A(n)$ agree for every sufficiently large $n \ge 1$. 




Next, we define a process $\XX^*(\ff)$ on each of the 

To define the coupling 
.


Here in the conditional probabilities 
%:= \P\big(\XX^*_v = \s \ba \XX^*_{\pa v} = \bs {\s'}\big)$$


$\{\k^*_v\}_{v \in V}$ as follows.


Then, we let $\pdo = \{\pdo_v\}_v$ denote an iid Bernoulli process with $\P(\pdo_v = 1) = p_0$.

We now construct a coupling of $\XX'$ and $\pdo$ such that $\pdo$ dominates $\XX'$ in the sense that $\XX' \su \pdo$ a.s. To achieve this goal, we first set $\XX_v' = 0$ if $\pdo_v = 0$. Next, conditioned on $\pdo$, we define $\XX'$ independently in each of the $\pdo$-occupied connected components. More precisely, if $A$ is such a component, we set  \begin{align}
	\label{eq:coup}
	P\big(\XX_A' \in B\big):= p^{-|A|} \P\big(\XX_A \in B \b \ba \XX_\big),
\end{align}

We now show that $\XX$ and $\XX'$ have the same distribution.

\bel[Correctness of coupling]
\label{lem:coup}
The processes $\XX$ and $\XX'$ have the same distribution.
\enl
\bep
Let $\om \in\{0, 1\}^V$ be arbitrary. Then, we compute $\P(\XX' = \om)$. Then, by definition
$$\P(\XX' = \om) = \sum_{\om' \supset \om}\P(\XX' = \om,\, \pdo =\om')$$
Now, let $A_1, \dots, A_N$ be the connected components of $\om_1'$. Then, 
$$\P(\XX' = \om) = \sum_{\om' \supset \om}\P(\pdo = \om') p^{-|\om'_1|}\prod_{i \le N}\P\big(\XX_{A_i} = \om_{A_i}\ba \XX_{\pa A_i} = 0\big).$$
Now, we note that by the spatial Markov property, we have that 
$$\prod_i \P\big(\XX_{A_i} = \om_{A_i}\ba \XX_{\pa A_i} = 0\big) = \P\big(\XX = \om\big) \P\big(\XX_{\om'_0} = 0\big) ^{-1}$$
\enp

We will use Lemma \ref{lem:sd} in the case where $p_0 < p_c$ is smaller than the critical probability of percolation on $G$. Then, we can realize the process $\XX$ in a two-step procedure. 
First, we generate the clusters of the independent process $\pdo$. Then, we generate the Gibbs process in each of these clusters separately. This two-step approach has the key advantage that the dependencies of the Gibbs process are confined to the clusters of $\pdo$.   We often call $\pds = (\Psi, \pdo)$ also the augmented Gibbs process. We now formalize this idea  by proving that the conditioned augmented process also satisfies a spatial Markov property.

\bel[Conditional spatial Markov property]
\label{lem:mark}
Let $A \su V$ and $B \su \{0, 1\}^A$. Then, 
\begin{align*}
	\P\big(\Psi_A \in B\ba \pdo, \Psi_{\hat A}\big)	\one\{\pdo_A = 0\} = \P\big(\Psi_A \in B\ba \pdo, \Psi_{\partial A} = 0\big)\one\{\pdo_A = 0\}
\end{align*}
\enl
\bep

\enp



The key implication of  Lemma \ref{lem:sd} is a a local simulation of $\XX$ 
allows to generate 


